Automatic Categorization of GitHub Actions with Transformers and Few-shot Learning

In the GitHub ecosystem, workflows are used as an effective means to automate development tasks and to set up a Continuous Integration and Delivery (CI/CD pipeline). GitHub Actions (GHA) have been conceived to provide developers with a practical tool to create and maintain workflows, avoiding reinventing the wheel and cluttering the workflow with shell commands. Properly leveraging the power of GitHub Actions can facilitate the development processes, enhance collaboration, and significantly impact project outcomes. To expose actions to search engines, GitHub allows developers to assign them to one or more categories manually. These are used as an effective means to group actions sharing similar functionality. Nevertheless, while providing a practical way to execute workflows, many actions have unclear purposes, and sometimes they are not categorized. In this work, we bridge such a gap by conceptualizing Gavel, a practical solution to increasing the visibility of actions in GitHub. By leveraging the content of README.MD files for each action, we use Transformer--a deep learning algorithm--to assign suitable categories to the action. We conducted an empirical investigation and compared Gavel with a state-of-the-art baseline. The experimental results show that our proposed approach can assign categories to GitHub actions effectively, thus outperforming the state-of-the-art baseline.

==> src/Approach.tex <==

We use multi-category classification.

%\section{Data Collection} \label{sect:approach}
%
%
%
%
%
%%\section{\GS: Summarization of \GH \RM} \label{sect:approach}
%
%The workflow of our \GS is presented in Fig~\ref{fig:workflow}, including three main phases, \ie \textit{Data Collecting}, \textit{Summarizing}, and \textit{Generating \& Evaluating}. Firstly, \RM data is fetched from real open-source projects in \GH by means of the \textit{Data Collecting} phase. After that, the data is pre-processed and fed to the selected pre-trained model for further training in the \textit{Summarizing} phase. Finally, %we perform \textit{Generator} component to 
%summaries for elements in test dataset are generated, and evaluated. %using the ROUGE score. %The three phases are described in detail as follows.
%
%
%
%
%
%
%\subsection{Labeling process}
%
%Follow an Active learning strategy: 
%\begin{enumerate}
%	\item Training a model on the available dataset D.
%	\item Use the trained model to select hard data for labeling.
%	\item Selected set D' is labeled by annotators
%	\item Combine 2 set: D = D + D'. Go to step 1.
%\end{enumerate}
%
%
%\begin{figure*}[h!]
%	\includegraphics[width=0.6\textwidth]{figs/activate_learning.png}
%	\centering
%\end{figure*}
%
%
%\subsection{Labeling guideline}
%
%- Labeling data based on \textbf{COMMENT} and \textbf{CODE} in the source code.
%
%
%- Labeling steps:
%\begin{enumerate}
%	\item Give each student an Excel file. Each row contains a comment along with code. \newline Note: you may see some comments does not appear in the code and usually start with "/*", this is because it is a comment block before the function and indicates the general content of the function.
%	\item After carefully reading it, you should select what type of self-admitted technical debt the source code should be classified as. To do this, just choose one of the 6 labeled in the droplist of \textbf{classification} column.
%	\item After classifying a source code, you must set the value of \textbf{isFinised} column to TRUE.
%	% \item There is no time limit to complete your task. If you desire to pause the classification process you can close your web browser and restart your work later by repeating steps 1 and 2.
%\end{enumerate}
%
%





%\begin{figure}[!h]
%	\centering
%	\vspace{-.2cm}
%	\includegraphics[width=0.48\textwidth]{figs/GitSum_Workflow.pdf}
%	\caption{The \GS workflow.}
%	\label{fig:workflow}
%	\vspace{-.4cm}
%\end{figure}

% The ``\verb|acmart|'' document class requires the use of the
% ``Libertine'' typeface family. Your \TeX\ installation should include
% this set of packages. Please do not substitute other typefaces. The
% ``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
% as they will override the built-in typeface families.



%\subsection{Data fetching} \label{sec:DataCollecting}


% \PN{@Juri: Please help me with this section. Thanks!}


%This components interacts with \GH to collect training data. 

%Mining repositories is a process of 


%========================================
%The extraction of data from \GH repositories can be done in different ways, including \GH API, \GH snapshots, and \GH GraphQL. %
%Using the \GH GraphQL\footnote{\url{https://docs.github.com/en/graphql}}, we crawled repositories to provide input for the evaluation.
%We opted for \GH GraphQL API to crawl repositories to provide input for the evaluation, as it offers a more flexible, efficient, and robust way of querying data compared to the other alternatives. 
%While there may be some trade-offs, such as a steeper learning curve and the need for additional tooling, the benefits of using the GraphQL API can be significant. In particular, GraphQL API provides a more flexible way of querying data compared to the REST API. With GraphQL API, we can request exactly the needed data, without getting any redundancy. This can reduce the amount of data returned, saving bandwidth and improving performance. %GraphQL API allows us to perform 
%complex queries requiring multiple REST API calls with the REST API. %With GraphQL API, you can obtain all the data you need in a single query, improving efficiency and reducing the number of round trips to the API. 
%========================================
%
%GraphQL API allows for a strongly typed schema that defines the available data and the relationships between the data. %This schema enables a better tooling and a more efficient development process than the REST API, which relies on documentation to understand the available data. %Moreover, GraphQL API provides real-time updates through the use of subscriptions. 
%A search query can be executed to perform a repository search on \GH using GraphQL. The search facility requires three parameters, including a \textit{query} to search for, the \textit{type} of entity to search for, and the \textit{number} of requested results (max 100).
%\vspace{-.2cm}
%\begin{lstlisting}[language=json,firstnumber=1,caption=Search parameters.,label={lst:example},numbers=none]
%query:"topic:'<featured-topic>' stars:>500'# Introduction' in:readme", type: Repository, first:100
%\end{lstlisting}
%
%As shown in Listing~\ref{lst:example}, we considered repositories with more than 500 stars to avoid toy or dummy ones. Since the \GH Search API provides up to 1,000 search items, we used a python script to perform searches iteratively by varying the topics query element. Those topics are extracted for \GH featured-topic list.\footnote{\url{https://github.com/topics}} The script iterates among the result pages if needed. Because we are interested in summarizing \RM files, we restrict the results to repositories that include structured \RM files. The response to this query contains information about the repositories that match the search criteria, such as their name, description, number of stargazers, and the login of the repository owner.

%This information is specified in the query by defining the desired fields in the ... on Repository section.
%The resulting query can be executed by sending a POST request to the \GH GraphQL API endpoint, with the query included in the request body and the access token provided in the Authorization header.




%
%
%\subsection{Summarizing}
%
%%\subsection{The BART pre-trained model}
%% T5 brief introduction \\
%
%% \PN{We will use both BART and T5 as the prediction engine.}
%
%% \PN{I am going to restructure and revise this section. Currently, it is lengthy.}
%
%
%\vspace{.1cm}
%\noindent
%$\rhd$~\textbf{BART.} %For our summarization tasks of README.MD, we use BART (Bidirectional Auto-Regressive Transformer) as our baseline. 
%This is a standard sequence-to-sequence Transformer architecture %, which was firstly
%developed by Lewis \etal \cite{bart2020}. Built on top an encoder-decoder architecture, BART has demonstrated its ability to achieve state-of-the-art (SOTA) results in several summarization tasks. Furthermore, it was fine-tuned as standard Seq2Seq models in order to provide a quick solution for various sequence-to-sequence learning problems.  It can be considered as generalizing BERT (due to the bidirectional encoder), GPT (with the left-to-right decoder), and many other more recent pretraining schemes. But following GPT, GELU is used as the activate function in BART instead of ReLU. %. %In the original paper, the experimental results performed on two news summarization datasets show that 
%%BART outperforms all existing approaches, yielding  a promising performance in solving summarization problems.
%%Technically, BART is applied several techniques, such as token masking. token deletion, text infilling, sentence permutation, and document rotation. 
%%BART is trained by
%%BART has been pre-trained in large English corpora including 160GB of uncompressed text, interfering text with an arbitrary noising function, and learning a model to reconstruct the original text.
%
%% Detail about the used BART configuration...
%
%
%%=======================================================
% %This format makes T5 fit for various tasks, such as translation, question answering, summarization, etc.
%% Technically, 
%
%
%
%\vspace{.1cm}
%\noindent
%$\rhd$~\textbf{T5.} Text-to-Text-Transfer-Transformer (T5) was firstly introduced by Raffel \etal \cite{t52019}, and it becomes one of the state-of-the-art pre-trained models, which has shown to obtain a promising performance in solving NLP tasks. T5 is based on a Transformer architecture using a text-to-text approach as its input and output are always presented in text strings, and trained in a high quality pre-processed English corpus with 700GB in size~\cite{t52019}. T5 is pre-trained with the same objective to BERT \cite{bert2018}, following the concepts of Masked Language Models. Masked Language Models are Bidirectional models in which the representation of a word is derived from both the left and the right of its context. %The subtle difference is that T5 replaces multiple consecutive tokens with a single mask keyword, while BERT uses mask token for each word. 
%


% T5 uses relative scalar embeddings. Encoder input padding can be done on the left and on the right.
% As you can see from the above diagram, the Original text is transformed into Input and Output pairs by adding perturbations to it. Since the final objective is to have trained a model that inputs text and outputs text, the targets were designed to produce a sequence, unlike BERT, that tries to output one word (itself) through final feed-forward and softmax at the output level.
% How is T5 applied in this work?\\
% T5 has demonstrated outstanding performance with state-of-the-art results on many NLP benchmarks while being flexible enough to be fine-tuned to a variety of important downstream tasks. From that point of view, 

% We apply T5 to our work by fine-tuning it on a domain-specific README.MD dataset accrued from \GH. 


%=======================================================

%  For every text sequence in its input, the BERT encoder outputs an embedding vector for each token in the sequence as well as an additional vector containing sentence-level information.
% Once we get the token and sentence-level representation of an input text sequence, a decoder needs to interpret these to map with the output target.

%
%\begin{table}[!h]
%	\centering
%         \small
%         \footnotesize
%         \vspace{-.25cm}
%	\caption{Details of the base BART and T5.} 
%        \vspace{-.2cm}
%	\begin{tabular}{|l|c|c|} \hline %\toprule
%		\textbf{Pre-trained model} & \textbf{BART} & \textbf{T5}  \\
%        \hline    
%        \textbf{Development team}    &  Facebook     & Google  \\
%        \hline
%		\textbf{\# encoder-decoder layers}      & 6    & 12  \\ 
%        \hline
%        \textbf{Embedding size} & 1,024    & 512  \\ 
%        \hline
%          \textbf{Beam size}      & 4    & 4  \\ 
%          \hline
%       \textbf{Length penalty}      & 1.0    & 1.0  \\ 
%        \hline
%        % \textbf{Vocabulary size}      & 50,265    & 32,128  \\ 
%        % \hline
%		\textbf{\# parameters} & 140M    & 220M \\ 
%        % \hline
%		% \textbf{Pre-trained in datasets} & English Wikipedia  &  C4 \cite{c4} \\ 
%  %        & and BookCorpus \cite{1} &    \\ 
%        \hline %\bottomrule
%	\end{tabular}	
%	\label{tab:bart_t5_base_version}
%     \vspace{-.35cm}
%\end{table}



% \begin{table}[!h]
% 	\centering
% 	\caption{Details of the base BART model.}  %N/A implies not applicable.
% 	%	\footnotesize
% 	\begin{tabular}{|l|c|} \hline %\toprule
% 		\textbf{Pre-trained model} & \textbf{BART} \\
%         \hline    
%         \textbf{Development team}    &  Facebook   \\
%         \hline
% 		\textbf{\# encoder-decoder layers}      & 6  \\ 
%         \hline
%         \textbf{Embedding size} & 1,024  \\ 
%         \hline
%           \textbf{Beam size}      & 4   \\ 
%           \hline
%        \textbf{Length penalty}      & 1.0  \\ 
%         \hline
%         % \textbf{Vocabulary size}      & 50,265    & 32,128  \\ 
%         % \hline
% 		\textbf{\# parameters} & 140M   \\ 
%         % \hline
% 		% \textbf{Pre-trained in datasets} & English Wikipedia  &  C4 \cite{c4} \\ 
%   %        & and BookCorpus \cite{1} &    \\ 
%         \hline %\bottomrule
% 	\end{tabular}	
% 	\label{tab:bart_t5_base_version}
% \end{table}





% \PN{Should we have a module for tokenizing text?}

% We utilize pre-trained BART as our underlying model. 

% is adopted for the \RM summarization task. 
%The source sequence is the \RM, and the target sequence is the description that goes along with it. 
%
%\input{example.tex}
%
%In this implementation, we adopted T5 and the base version of BART as the classification engine. We set all the hyper-parameters values as the default configuration. Details about the BART and T5 recommendation engines are depicted in Table~\ref{tab:bart_t5_base_version}. We continuously trained on \RM files and their descriptions. For every \RM and its description in the training dataset that could be considered as a pair of source sequence and target sequence, they are tokenized into token vectors by using the tokenizier going along with each pre-trained model. Afterward, the achieved token vectors of the source sequence and the target sequence are fed to the models to update weights.\footnote{The fine-tuning script and other materials related to our work are provided in the replication package.} 
%
%
%
%
%\subsection{Generating \& Evaluating}
%In this phase, %we investigate the performance of \GS on our summarization task after fine-tuning. 
%the model is used to the prediction engine, which has been trained with several training repositories. %generate summaries for testing repositories. 
%\RM files of testing repositories are  used as input to generate summaries. The real label of each testing instance is removed to use as ground-truth data. The generated summaries are then compared with the real ones in the ground-truth data to evaluate the performance. In reality, \GS should be trained with a lot of repositories to provide predictions for those without any ``About'' description.



%and compare the generated results to the real description. %We use the ROUGE metrics in comparing two sequences.




==> src/Discussion.tex <==
\section{DISCUSSION}~\label{sec:discussion}
 %AND THREATS OF VALIDITY

In this section, we discuss various implications ... Moreover, we also highlight the threats to validity of our findings.

\subsection{Implications}






\subsection{Threats to validity}

%\vspace{.1cm}
%\noindent
%$\rhd$~\textbf{Internal validity.} 

\begin{itemize}
    \item \textbf{Internal validity.} This concerns how well our evaluation resembles real-world scenarios. In the evaluation, we crawled data from \GH, and for the testing projects, we removed their real descriptions, and saved as ground-truth data. %This simulates a real development scenario where we need to recommend summary for repositories using their \RM. %adopted existing datasets~\cite{missing} manually curated and classified. The quality of the curated data depends very much on the evaluators' expertise. We anticipate that comments might be miss-classified, thus negatively impacting the overall prediction performance. 	
    \item \textbf{External validity.} This is related to the generalizability of the findings outside this study. %We attempted to mitigate the threats by evaluating \GS using different experimental configurations to simulate real-world scenarios. Since there exists no approach with the same purpose, \IT--a tool for generation of titles for bug reports--was chosen as the baseline. %for comparison. %For the comparison with the baseline, we used the original implementation published by the authors. 
%we extracted the results from the original paper and executed ... on the same datasets, using identical experimental settings. %Moreover, our proposed tool is applicable to other languages rather than Java, such as C++, Python, or R provided that there are proper tools to extract comments from source code to supply input for ...
    \item~\textbf{Construct validity.} This threat is related to the experimental settings to compare %\GS with \IT. To aim for a reliable comparison, we used the original implementation of \IT made available by its authors,\footnote{\url{https://github.com/imcsq/iTAPE}} keeping the internal design unchanged. Moreover, we tried to employ the same settings to experiment with both systems.
%\end{itemize}

\end{itemize}










% \subsection{Synergy of \tool and existing techniques}~\label{sec:combine}% 
% As discussed in Section~\ref{sec:rq2} and~\ref{sec:rq3}, we found that \tool excels in head and mid labels but performs worse than ZestXML in tail labels, which rarely happened.  In this section, we discuss the possibility of a synergistic approach of \LG and existing approach for better \GH topic recommendation. Particularly, we design a synergistic approach by combining top-3 predictions from ZestXML and top-5 predictions from \LG for the final top-8 predictions. The rationale behind this design is: (1) we observe that \LG and ZestXML show the optimal effectiveness on top-5 and top-3 predictions, respectively, and (2) we avoid bias on tail labels, which rarely happens and may harm performance. Table~\ref{tab:combine} illustrates the effectiveness of the synergistic approach compared to \LG and ZestXML.
% \begin{table}[h]
% \caption{The effectiveness (F1-score) of synergistic approach of ZestXML and \LG.}~\label{tab:combine}
% \begin{tabular}{l|cc|c}
% \hline
%      & \multicolumn{1}{l}{\textbf{ZestXML}} & \multicolumn{1}{l|}{\textbf{\tool}} & \multicolumn{1}{l}{\textbf{Synergistic approach}} \\ \hline
% \textbf{Head} & 0.340                        & \textbf{0.536}              & 0.532                         \\ 
% \textbf{Mid}  & 0.341                        & 0.473                       & \textbf{0.489}                \\ 
% \textbf{Tail} & 0.193                        & 0.079                       & \textbf{0.267}                \\ \hline
% \textbf{All}  & 0.337                        & 0.525                       & \textbf{0.526}                \\ \hline
% \end{tabular}
% \end{table}

% Overall, we can see that the synergistic approach outperforms ZestXML and \LG in mid and tail labels and only shows a slight decrease in performance in head labels. Consequently, the approach shows the best performance in whole labels. While the improvement is very marginal, we can see that this synergistic approach is more reliable than ZestXML and \LG as it offers consistent performance over different subsets of labels. We encourage future works to explore this direction for better \GH topic recommendation techniques. 

% \subsection{Threats to Validity} 
% \subsubsection{Internal Validity.} This threat refers to possible flaws in our experiments and implementations. We have carefully checked the correctness of our implementation. We also published our source code along with trained models~\cite{GitHubTopicRecSys} %at\footnote{} 
% and presented detailed hyper-parameters for the training of considered models in Section~\ref{sec:implementation}. Given these materials, other research can validate our results and findings. Therefore, we believe that there are minimal threats from this issue.  
% \subsubsection{Construct Validity.} This threat concerns the suitability of our evaluation. A source of these threats may stem from our evaluation metric. To minimize this threat, we employ well-known metrics, which are commonly used by prior studies~\cite{izadi2021topic,di2022hybridrec, lyu2023chronos, widyasari2023topic} for multi-label classification, including  Precision, Recall, and F1-score.

% \subsubsection{External Validity} This threat relates to the
% generalizability of our findings. Our experiments are conducted on the same dataset as prior work~\cite{widyasari2023topic}, crawled from \GH. This raises a concern about the external validity of our findings as they may not generalize beyond \GH repositories outside our dataset. However, we believe this threat is minimal as the dataset is exhaustively crawled from \GH and consists of a large number of data points, which ensure their diversity. 


==> src/Empirical_Evaluation.tex <==
\section{EMPIRICAL EVALUATION}  \label{sec:settings}

In this section, we present an empirical evaluation to study the performance of our proposed approach.

\subsection{Research Questions}
\label{sec:ResearchQuestions}

%In this work, 
A series of experiments was conducted to answer the following research questions:

\vspace{.2cm}
\noindent \rqone~This research question seeks to determine the efficacy of Pre-trained Language Models (PLMs) in generating titles for \SO posts and demonstrates for our choice, the CodeT5 model.
We evaluate five distinct PLMs, namely BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}, CodeT5~\cite{wang2021codet5}, CodeBERT~\cite{feng2020codebert} and UnixCoder~\cite{guo2022unixcoder}.
The first two models are designed for natural language processing, whereas the latter three are specialized in understanding and representing programming languages.
We applied the fine-tuning process to five pre-trained models--BART, T5, CodeT5, CodeBERT and UnixCoder--utilizing the benchmark datasets described in Section~\ref{sec:dataset}.
This process followed the configuration settings outlined by Liu et al.~\cite{liu2022sotitle}.
%, who previously fine-tuned the pre-trained T5 model for \SO post title generation. 
%Additionally, the outcomes from the fine-tuned T5 model in title generation for \SO posts were also sourced from their study.

\vspace{.2cm}
\noindent \rqtwo~In this question, we compare the performance of our proposed approach to the baseline works. We choose four recent state-of-the-art models for \SO post title generation including \texttt{Code2Que}~\cite{gao2021code2que}, \texttt{SOTitle}~\cite{liu2022sotitle}, \texttt{CCBERT}~\cite{zhang2022improving} and \texttt{M3NSCT5}~\cite{zhang2023diverse}, which have obtained a promising recommendation performance. 
%\textbf{DAVIDE: Is there any criteria used to list existing approaches in the following order? The same question applies to the order of the four references given in the previous sentence.MA: I change the above order to align with the following list, according the publishing year}

\begin{itemize}
    \item \textbf{\texttt{Code2Que}~\cite{gao2021code2que}:}
    Gao et al.~\cite{gao2021code2que} proposed the \texttt{Code2Que} model to generate Stack Overflow titles from code snippets. This model is underpinned by an LSTM encoder-decoder architecture, augmented with the integration of copy and coverage mechanisms. The copy component enhances the decoder’s ability to focus on relevant parts of the input, whereas the coverage strategy plays a crucial role in reducing unnecessary repetitions, thereby refining the output quality.
    \item \textbf{\texttt{SOTitle}~\cite{liu2022sotitle}:}
    Liu et al.~\cite{liu2022sotitle} fine-tuned the pre-trained T5 model on their collected \SO dataset. 
    They employed a multi-task learning architecture in which the description and code snippet of each \SO post were concatenated together for each programming language but followed a simultaneous training process. 
    This multi-task learning strategy facilitates information sharing across different programming languages, thereby improving each other's performance.
    \item \textbf{\texttt{CCBERT}~\cite{zhang2022improving}:}     
    The model was proposed by Zhang et al.~\cite{zhang2022improving}, employing CodeBERT to encode both the code snippets and question descriptions. It is further enhanced by integrating a copy attention layer to refine the quality of the generated output.
    \item \textbf{\texttt{M3NSCT5}~\cite{zhang2023diverse}:}
    This model was developed to generate multiple post titles from the given code snippets. The pre-trained CodeT5 model was utilized as the backbone, combined with the maximal marginal ranking strategy to select the most relevant and diverse titles from multiple generated samples.
\end{itemize}

It is worth mentioning that all the baseline models mentioned earlier--except for \texttt{Code2Que}--are predominantly fine-tuned pre-trained language models for generating post titles. Notably, \texttt{SOTitle} and \texttt{CCBERT} are bi-modal models, whereas \texttt{Code2Que} and \texttt{M3NSCT5} rely solely on code snippets. 
For a fair comparison with \tool, % our proposed method, 
we fine-tuned these models using code snippets and question descriptions, following the methodology established by Liu et al~\cite{liu2022sotitle}.

\vspace{.2cm}
\noindent \rqthree~In our research, we implemented two strategies to enhance the \SO post title generation model: a Self-Improvement approach during training and a Post-Ranking method for selecting the most pertinent title for a given question body. This research question aims to assess how each of these components contributes to the overall efficacy of the proposed model. 

\vspace{.2cm}
\noindent \rqfour~
\correct{rephrase or rewrite}{Motivation. 
There exist some disadvantages to automatic evaluation measures. For example, the text overlap-based measures used in our study may not effectively reflect the similarity between the generated question title and the ground-truth question title from a semantic perspective (Hu et al 2020). Therefore, we want to conduct a human study to evaluate the competitiveness of SOTitle+ in this RQ. (Copy from sotitle+ ) In the previous study have show that the overlap-based measures, While this provides a simple and general measure, it fails to account for meaning-preserving lexical and compositional diversity (Copy from bert score) For the problem of the generated title with a similar semantic but dissimilar description, we should design more effective performance measures, since currently used measures (such as BLEU (Papineni et al., 2002), ROUGE (Lin, 2004)) cannot solve this problem(Copy from TitleGen-FL: Quality prediction-based filter for automated issue title generation)}

\vspace{.2cm}
\noindent \rqfive~
\correct{rewrite}{Recently, LLMs (Brown et al 2020) (e.g., ChatGPT) have attracted great attention and
achieved promising performance for many software engineering tasks, such as program repair (Xia and Zhang 2023) and code generation (Liu et al 2023a). In this subsection, we want to investigate the effectiveness of using ChatGPT in the SOQTG task and whether SOTitle+ can outperform ChatGPT on the posts related to Go and Ruby. Specifically, for ChatGPT, we use OpenAI official API17 and the hard prompt introduced in Section 2.2.1 since ChatGPT does not support hybrid prompt. For SOTitle+, we directly use the model trained for answering RQ1. Notice both SOTitle+ and ChatGPT are not trained on the corpus related to Go and Ruby. Therefore, they are compared in the zero-shot scenario.(Copy from Sotitle+)}

\subsection{Dataset}\label{sec:dataset}
In this research, we use a benchmark dataset from a previous study~\cite{liu2022sotitle}, comprising \SO posts in four different languages: Java, C\#, Python, and JavaScript (JS), which are among the most popular programming languages. Each post includes a brief title, a descriptive question, and a code snippet. The dataset encompasses 284,298 posts across these four languages, divided into training, validation, and testing subsets. For each language, there are 60,000 and 5,000 posts for training and testing, respectively. Detailed statistics of the benchmark dataset are shown in Table~\ref{tab:dataset}.

\begin{table}[t]
    \centering
    \caption{Statistics of the benchmark dataset.}
    \begin{tabular}{lccc}
    %\toprule
    \hline
         \textbf{Language} &  \textbf{Training}  & \textbf{Validation}& \textbf{Testing} \\
         \hline
        %\midrule
          Java & 60,000 & 3,959 & 5,000 \\
          C\#  & 60,000 & 6,817 & 5,000 \\
          Python & 60,000 & 7,742 & 5,000 \\
          JavaScript & 60,000 & 5,780 & 5000 \\
          \hline
          \textbf{Total} & 240,000 & 24,298 & 20,000 \\
          \hline
    \end{tabular}
    \label{tab:dataset}
\end{table}

% We started with data provided by a prior work~\cite{widyasari2023topic}, which has already been split into train and test sets of 17,018 and 4,225 repositories, respectively. As stated in Section~\ref{sec:preprocessing}, to ensure the quality of our dataset, we focus on \GH's featured topics. The result is a dataset with total 15,262 repositories and 665 unique labels. We extract randomly 1,000 repositories from the training data to create a validation set. The dataset now contains 11,282 training, 2,980 testing and 1,000 validation repositories. The statistics of our training and testing datasets are shown in Table ~\ref{tab:dataset}.
  
\subsection{Evaluation Metrics}\label{sec:metric} 
To evaluate the accuracy of the generated Stack Overflow post titles, we utilize ROUGE metrics~\cite{lin2004rouge}. Specifically, we calculate ROUGE-1 (R-1), ROUGE-2 (R-2), and ROUGE-L (R-L), which have been extensively used in prior studies for tasks involving text generation and summarization~\cite{liu2022sotitle,gao2021code2que,zhang2022improving,zhang2023diverse}. 
ROUGE--1 and ROUGE--2 rely on 1--grams and 2--grams, respectively, whereas ROUGE--L focuses on the longest continuous sequence.
The recall, precision, and F1-Score for the ROUGE-$k$ metrics are defined as shown in Equations~\ref{eq:recall}, \ref{eq:precision}, and \ref{eq:f1}.

\begin{equation}
    \label{eq:recall}
    \text{Recall}_{rouge-k} = \frac{\#\text{overlapped\_}k\text{\_grams}}{\#k\text{\_grams} \in \text{gold summary}}
\end{equation}

\begin{equation}
    \label{eq:precision}
    \text{Precision}_{rouge-k} = \frac{\#\text{overlapped\_}k\text{\_grams}}{\#k\text{\_grams} \in \text{generated summary}}
\end{equation}

\begin{equation}
    \label{eq:f1}
    \text{F1-Score}_{rouge-k} = 2 \times \frac{\text{Recall}_{rouge-k} \times \text{Precision}_{rouge-k}}{\text{Recall}_{rouge-k} + \text{Precision}_{rouge-k}}
\end{equation}
where the {\it gold summary} refers to the original title of the SO post while the {\it generated summary} denotes the title generated by the underlying model.
The {\it overlapped\_$k$\_grams} indicates the $k$\_grams which appears in both the gold summary and the generated one. 
The recall metric calculates the proportion of $k$-grams in the reference summary that are included in the generated summary, whereas precision determines the proportion of $k$-grams in the generated summary that are present in the gold summary. The F1-Score represents a balance between the recall and precision metrics.
This study adopts the F1-Score as the primary evaluation metric, in line with prior research~\cite{zhang2022improving,zhang2023diverse}.
Additionally, we employ the recall metric to compare how different models perform in aligning the generated summaries with the reference ones in terms of similarity~\cite{liu2022sotitle}.


% The experiments aim to evaluate the effectiveness of our proposed approach and state-of-the-art baselines in \GH topic recommendation using three evaluation metrics, \ie Precision@K, Recall@K, and F1-score@K, which have been widely utilized for the same purpose~\cite{widyasari2023topic, lyu2023chronos}. Particularly, given the top-K predictions for a repository, all metrics are calculated globally based on the total count of true positives, false negatives, false positives defined as follows:
% \begin{itemize}
%     \item \textbf{True Positives (TP):} a topic is suggested to a repository by a recommender, and it is an actual topic of the repository. 
%     \item \textbf{False Positives (FP):} a topic is suggested to a repository by a recommender, but it does not belong to the repository. 
%     \item \textbf{True Negatives (FP):} a topic is not suggested to a repository by a recommender, and it does not belong to the repository. 
%     \item \textbf{False Negatives (TP):} a topic is not suggested to a repository by a recommender, but it is an actual topic of the repository. 

% \end{itemize}

% \textbf{Precision} measures how \textit{precise/accurate} the suggested topics are. It is calculated by the ratio of true topics (true positives) over the total number of predictions. More formally,
% \begin{equation}
%     P = \dfrac{TP}{TP+FP}
% \end{equation}
        
% \textbf{Recall} measure how \textit{complete} are suggested topics. It is calculated by the ratio of true topics suggested (true positives) by a recommendation system over the total number of actual topics. 
% \begin{equation}
%     P = \dfrac{TP}{TP+FN}
% \end{equation}

% \textbf{F1-score} is a harmonic mean of the precision and recall, seeking the balance between these metrics:
% \begin{equation}
%     F1 = \dfrac{2 \times (P \times R)}{P + R}
% \end{equation}
        
% In this work, we leverage Micro-F1~\cite{wu-etal-2019-learning,lipton2014thresholding}, which takes label imbalance into account. 


\begin{table*}[htp]
    \centering
    \small
    \caption{Performance of Pre-trained Models (PLMs) including BART, T5, CodeBERT, CodeT5, and UnixCoder in title generation for \SO Posts.}
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
        \hline
        %\toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Java}} & \multicolumn{3}{c|}{\textbf{C\#}} & \multicolumn{3}{c|}{\textbf{Python}} & \multicolumn{3}{c|}{\textbf{JavaScript}} & \multicolumn{3}{c}{\textbf{Average}}\\
        \cline{2-16} & R--1& R--2& R--L& R--1& R--2& R--L& R--1& R--2& R--L& R--1& R--2& R--L & R--1 & R--2 & R--L\\ 
        \hline
        \textbf{T5}$_{256+256}$ & 26.49	&9.80	&24.60&	26.94&	10.76&	25.17& 29.00&	10.79&	26.70&	28.53&	10.77&	26.47& 27.74&	10.53	&25.74\\
        \textbf{T5}$_{512}$ & \textbf{28.72}&	\textbf{11.14}&	\textbf{26.59}&	29.03&	12.07&	27.21& 31.39&	12.37&	28.87&	30.96	&12.65	&28.80& 30.03	&12.06	&27.87 \\
        
        \textbf{BART} & 28.40&10.96&	26.35&		28.48&	11.80&	26.72& 31.25&	12.29&	28.79&	30.62&	12.16&	28.51& 29.69	&11.80&	27.59\\
        
        \hline
        \textbf{CodeBERT} & 25.22	&9.31& 	23.62& 	25.17	& 10.28& 	23.85&  28.16& 	10.75	& 26.36	& 27.49& 	10.67& 25.85& 26.51&	10.25&	24.92\\
        \textbf{UnixCoder} & 25.28	&9.34	&23.58&	25.54&	10.49	&24.17 &27.49	&10.00	&26.10	&27.84&	10.66&	26.08& 19.73	&7.65&	18.52  \\
        \textbf{CodeT5} & 28.64 & 11.10&26.53 & \textbf{29.24} & \textbf{12.38} & \textbf{27.31} &\textbf{31.94} & \textbf{12.71} & \textbf{29.40} & \textbf{31.23} & \textbf{12.74} & \textbf{29.16} & \textbf{30.26} &\textbf{12.23}&\textbf{28.10} \\
        \hline
        %\bottomrule
    \end{tabular}      
    \label{tab:result_PLMs}
\end{table*}


\subsection{Implementation Details}\label{sec:implementation}
The implementation of \tool utilizes the Transformer library\footnote{\url{https://github.com/huggingface/transformers}} and is based on the checkpoint of the pre-trained CodeT5--base model, which features 12 layers for both encoder and decoder, each with a hidden size of 768.
The input sequences are tokenized using the Byte-Pair Encoding algorithm, characterized by a vocabulary size of 32,100.
These sequences are either truncated or padded to a maximum length of 512. 
The batching is carried out with a size of 4.
We employ the \texttt{AdamW} optimizer, with a default learning rate of $5e^{-5}$ for both the initial fine-tuning and the self--improvement stages. 
The model training lasts 8 epochs during the fine-tuning stage and 4 epochs in the self--improvement phase. We set the number of title candidates to 20 and 30 for the self--improvement and post--ranking processes, respectively.

For other Pre-trained Language Models including BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}, CodeBERT~\cite{feng2020codebert} and UnixCoder~\cite{guo2022unixcoder}, the parameters are initialized from \texttt{bart-base}, \texttt{t5-base},  \texttt{codebert-base} and \texttt{unixcoder-base-nine}.
All of the above models can be found on HuggingFace.\footnote{\url{https://huggingface.co/models}} All of our experiments have been carried out on PyTorch %, and are conducted 
on a single GPU RTX 2080 Ti with 12GB RAM. The evaluation metrics have been implemented using the \texttt{rouge} library.\footnote{\url{https://github.com/pltrdy/rouge}}

% We implement \tool  with the Transformer-2 library~\footnote{} and the pre-trained model checkpoint 3 of CodeT5-base version which has 12 encoder layers and 12 decoder layers with a hidden size of 768.
% The input sequences are tokenized using Byte-Pair Encoding algorithm, whose vocabulary size is 32,100 then truncated or padded to a maximum length of 512 and batched with batch size 4. The optimizer is AdamW. The default learning rate for the fine tuning stage and self improvement stage is 5e-5. All of our experiments are carried out using one GPU RTX 2080 Ti 12GB RAM. The model is set to train for 8 epochs on fine tuning stage and 4 epochs on self improvement stage. On the ranking stage we set the top-p sampling to 0.9 and top-k sampling to 5 for generate number of candidates. 
% The number of candidates in self-improvement stage and post ranking stage is set to 20 and 30, respectively.
% For the finetuning Unixcoder, Codebert we use the script release in here() , the Bart model was finetuned using the cript provide by hugging face. 
% The AutoModelForSequenceClassification backbone\footnote{\url{https://huggingface.co/transformers/v3.0.2/model_doc/auto.html}} in transformers library %\cite{} 
% was used to fine-tune our PLMs. The parameters for BERT \cite{bert} were initialized using the bert-base-uncased pretrained model. For RoBERTa \cite{roberta}, BART \cite{lewis2020bart}, and ELECTRA \cite{electra}, the parameteres were initialized from roberta-base, bart-base, and electra-base-discriminator models. All of the above models can be found on HuggingFace.\footnote{https://huggingface.co/models} Among them, bert-based-uncased and electra-base-discriminator follow the base BERT architecture with 110M parameters, while bart-base and roberta-base have 139M and 125M parameters respectively. The PLMs are fine-tuned using one Tesla V100 GPU which takes between 6 to 10 minutes for one epoch.
% The input sequences are truncated or padded to a maximum length of 512 and batched with batch size 32. The optimizer is AdamW with a weight decay of 0.01. The default learning rate for BCE models is 1e-5, but for models using DB loss the learning rate is 1e-4. Others parameters of both BCE and DB loss functions follow existing work~\cite{wu2020distribution,huang2021longtail}. %'s implementations. 
% All of our experiments are carried out on PyTorch. 
% For the older baselines, TF-IDF+LR and ZestXML+LR, we reuse the preprocessing, training and inference code from \cite{widyasari2023topic}. 
% During evaluation of the models, we acquire their top-k predictions on test set and calculate precision score, recall score, and micro F1 score using scikit-learn's functions \cite{scikit-learn}. 



==> src/Proposed_Solution.tex <==
\section{PROPOSED SOLUTION} \label{sec:Solution}


\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{img/Fig-architecture.pdf}
    \caption{The architecture of \tool.}
    \label{fig:Architecture}
    \vspace{-.2cm}
\end{figure*}


%\subsection{Overview}

This section describes our proposed approach to \SO post title generation--\tool--whose overall workflow is depicted in Figure~\ref{fig:Architecture}.
%We describe our proposed approach in 
There are three main stages as follows: \emph{fine-tuning, self-improvement} and \emph{inference}. During the fine-tuning stage, each SO post, comprising a question description and code snippet, is combined to form a bi-modal input.
%To address the out of vocabulary (OOV) issue, we utilize SentencePiece~\cite{kudo2018sentencepiece} for tokenizing these two modalities.
Our approach adopts a multi-task learning strategy, similar to previous studies~\cite{liu2022sotitle,zhang2023diverse,liu2023automated}, training the model simultaneously on various programming languages. We utilize a Pre-trained Language Model (PLM) as the backbone model and proceed with fine-tuning it on the \SO post dataset (see Section~\ref{sec:dataset}).

In addition to the conventional paradigm \emph{pre-training and fine-tuning}, our goal in the next stage is to boost the fine-tuned model’s performance by augmenting the training dataset. This enhanced dataset will be employed in a further fine-tuning stage. 
This process is referred to as the {\it self-improvement} technique~\cite{to-etal-2023-better}.
In the final inference stage, the model generates multiple candidate samples rather than producing just a single sample. From these, our proposed post-ranking method is designed to identify and select the highest quality title.
%
The next subsections explain in detail the constituent components of \tool. 

\subsection{Fine-tuning PLM with multi-modal inputs}
\label{sec:plms}
%The {\it pre-train then fine-tune} paradigm has been extensively employed in numerous Software Engineering (SE) tasks~\cite{}.
Fine-tuning using a Pre-trained Language Model for downstream tasks is a prevalent paradigm, extensively employed in numerous Software Engineering tasks~\cite{liu2023refining,chow2023beware,le2023invalidator}.
Our proposed method also follows this paradigm, utilizing the pre-trained CodeT5~\cite{wang2021codet5} model as the backbone model, then further updating its trainable parameters using a task-specific dataset consisting of pairs of SO post title and body.

Getting inspiration from previous research~\cite{zhang2022improving,liu2022sotitle,zhang2023diverse}, we create a bi-modal input for each Stack Overflow post by merging the code snippet with the question description. 
This combined representation is then tokenized using the Byte-Pair Encoding (BPE) method~\cite{sennrich-etal-2016-neural}, which has been integrated into the CodeT5 model. 
%with each pre-trained language model. For instance, the T5 model uses SentencePiece~\cite{kudo2018sentencepiece}, while CodeT5 employs Byte-Pair Encoding (BPE)~\cite{sennrich-etal-2016-neural}, and so on. 
This tokenizer is specifically designed to tackle the Out-of-Vocabulary (OoV) issues efficiently. We also explore a multi-task learning setting that enables training a shared model on multiple programming languages (PLs) simultaneously.
This approach allows for the reuse of model weights across various PLs, thereby reducing computational costs and enhancing the model's generalization capability~\cite{liu2020multi}. 
We prepend a prefix to the input sequence to inform the model about the specific language it is dealing with. 
Given a SO post, denoted as $\mathcal{X}$ which includes a sequence of code ($X_{code}$) and a sequence of question description ($X_{desc}$), the multi-modal input of $\mathcal{X}$ is formulated as shown in Equation~\ref{eq:input}.
\begin{equation}
    \label{eq:input}
    \mathcal{X} \,=\, <prefix> \oplus \,X_{desc}\, \oplus \,<code>\, \oplus\, X_{code}
\end{equation}
where $<prefix>$ denotes the programming language--specific prefix. For example, the prefix \texttt{JS} indicates the JavaScript programming language.
The special separator $<code>$ is used to distinguish between $X_{desc}$ and $X_{code}$.

%We fine-tune the pre-trained CodeT5 model to exploit the formatted SO posts with the aim of finding a set of parameters $\theta$ to minimize the negative log-likelihood of the target title $Y$ conditioned on the equivalent input sequence $\mathcal{X}$ from the training dataset, as follows.
We fine-tune the pre-trained CodeT5 model using formatted \SO posts. The goal is to identify a set of parameters $\theta$ that minimizes the negative log-likelihood of the target title $Y$  when conditioned on the corresponding input sequence $\mathcal{X}$ from the training dataset, given below.
\begin{equation}
    \label{eq:finetune}
    Y = \text{arg} \min\limits_{\theta} P(Y|\mathcal{X}; \theta)
\end{equation}
During the inference phase, we use the fine-tuned model in conjunction with the auto-regressive decoding method to get the predicted title $Y$ token by token.

\subsection{Self Improvement}
\label{sec:self}
This phase aims to enhance the performance of the Pre-trained Language Model for \SO post title generation through a data augmentation technique.

%Although PLMs have shown remarkable generalization to new tasks and greatly simplified engineering efforts as a single model can be used for multiple programming languages~\cite{liu2020multi}, most of them are auto-regressive sequence generation models which typically encounter exposure bias during training.
%Since auto-regressive sequence generation models often encounter exposure bias during training~\cite{wang2020exposure,guerreiro2023hallucinations}. 
Pre-trained Language Models have demonstrated impressive adaptability to new tasks, significantly reducing engineering efforts by allowing multi-modal modelling~\cite{wang2023large}.
However, auto-regressive sequence generation models typically encounter exposure bias during training phase~\cite{wang2020exposure,guerreiro2023hallucinations,to-etal-2023-better}.
This issue stems from a discrepancy between the training and inference stages.
To alleviate this bias, incorporating the model's own predictions during training can be 
\correct{@DA: It is important to use your own sentences} {We hypothesise that, while fine-tuned models may not achieve peak performance, PLMCs can produce reasonable outputs that can be regarded as high quality data because they have been pretrained on large scale datasets, and that such data can be leveraged as additional high-quality training data, this is copy from cite paper} 
beneficial~\cite{wang2020exposure}. This strategy allows the model to better manage its errors, leading to enhanced performance.
Inspired by this approach, we enhance our training dataset by incorporating predictions from the initially fine-tuned model. This augmented dataset is then employed to further refine the model through an additional fine-tuning stage.
%How to incorporate the prediction results

The self-improvement strategy is illustrated in Algorithm~\ref{alg:si}. 
Its input includes the initial training dataset $\mathcal{D}_t$, the number of generated candidates $k$ and the initially fine-tuned CodeT5 model ($\mathcal{M}_{\theta_f}$) which is characterized by the set of parameters $\theta_f$.
This procedure yields an enhanced version of the training dataset, denoted as $\mathcal{D}^{aug}_t$, which is then employed to fine-tune the model further.
For each pair consisting of an SO post and its corresponding ground truth title, $k$ title candidates are generated using the initially fine-tuned CodeT5 model. The candidate that achieves the highest ROUGE--L score (see Section~\ref{sec:metric}) when compared to the ground truth title is selected for inclusion in the augmented training dataset (Lines 2--9).

\begin{algorithm2e}[t]
\caption{Pseudo code of the Self--Improvement Process}
\label{alg:si}
\DontPrintSemicolon
\SetAlgoLined
%\KwResult{Write here the result}
\SetKwInOut{Input}{Input} 
\SetKwInOut{Output}{Output}
\Input{
    \begin{itemize}
        \item The fine--tuned model $\mathcal{M}_{\theta_f}$
        \item The original training dataset $\mathcal{D}_{t}$
        \item $k$ that denotes the number of generated candidates
    \end{itemize}
}
\Output{
\begin{itemize}
    \item The augmented training dataset $\mathcal{D}^{aug}_{t}$
    \item The new fine-tuned model $\mathcal{M}_{\theta_{f^*}}$
\end{itemize}
}

$\mathcal{D}^{aug}_{t} \leftarrow \emptyset$

\ForEach {$(\mathcal{X}_i,Y_i) \in \mathcal{D}_t$}
{
    $\mathcal{C}_i \leftarrow \emptyset$
    
	\ForEach {$j \in [1..k]$}
	{
		$\tilde{Y}_j \leftarrow \mathcal{M}_{\theta_f}\text{.predict}(\mathcal{X}_i)$
		
		$\mathcal{C}_i \leftarrow \mathcal{C}_i \bigcup \tilde{Y}_j$
	}

    $\tilde{Y}^*_i \leftarrow \text{arg}\max\limits_{\tilde{Y}_j \in \mathcal{C}_i} ROUGE_L(Y_i,\tilde{Y}_j)$
	
	$\mathcal{D}^{aug}_t \leftarrow \mathcal{D}^{aug}_t \bigcup (\mathcal{X}_i,\tilde{Y}^*_i)$
}

$\mathcal{M}_{\theta_{f^*}} \leftarrow \text{Fine-Tuning}( \mathcal{M}_{\theta_f},\mathcal{D}^{aug}_t)$

\Return{$\mathcal{D}^{aug}_t$ and $\mathcal{M}_{\theta_{f^*}}$}
\end{algorithm2e}

\subsection{Post Ranking}
\label{sec:ranking}
% Integrating ground truth with model predictions during training helps align it more closely with the inference process. 
% However, the use of maximization-based decoding strategies like beam search to determine the best sequence of tokens can introduce problems in text generation.
% As highlighted in prior research~\cite{holtzman2019curious}, this approach may result in text that either lacks coherence or is highly degenerate in some cases.
% Considerable research effort has been dedicated to tackling this issue, exploring various decoding techniques like top-k sampling, nucleus sampling, and others~\cite{holtzman2019curious,zhang2023diverse}. 
% Although these methods help in decreasing the repetition of tokens and enhancing diversity, the problem of hallucination persists.
% The main objective of this study is to focus on generating high quality title for SO posts, we aim to overcome the problem of hallucination through a post-ranking techniques during the inference stage.
Blending ground truth with model predictions during the training phase is essential for better alignment with the inference process. 
%However, employing maximization-based decoding strategies such as beam search for selecting optimal token sequences can lead to challenges in text generation of language models. According to previous studies~\cite{holtzman2019curious}, this method might produce text that is either incoherent or extremely degenerate. Significant research has been undertaken to address this, with investigations into various decoding strategies like top-k sampling and nucleus sampling~\cite{zhang2023diverse}. While these approaches reduce token repetition and improve diversity, the issue of hallucination remains unresolved. 
% The primary objective of our study is to create high-quality titles for \SO posts, with a specific focus on mitigating the issue of hallucinations through the use of a post-ranking method at the inference stage.
% Given that generating titles for posts is akin to summarizing into a short sentences, there is no requirement for the model to produce length text.
% % Consequently, the beam search algorithm remains an effective tool for this purpose.
Yet, in the text generation process, sequence generation models often utilize decoding strategies like beam search, greedy search, and nucleus sampling to select the best sequence of tokens~\cite{holtzman2019curious,zhang2023diverse}. %\textbf{DAVIDE: We should add some references for these strategies}. 
These methods’ inherent randomness can lead to significant variability in the quality of generated text. 
A widely used solution to this problem involves generating a range of sample candidates and then selecting the highest quality title among them~\cite{shi2022natural,inala2022fault}.

In this research, our goal is to generate high-quality titles for \SO posts, with a particular emphasis on addressing the issue of high variability in generation quality by implementing a post-ranking method during the inference phase. For each \SO post input $\mathcal{X}$, the model generates a set of $\mathbb{K}$ title candidates, denoted as $\mathcal{T} = \{T_1, T_2, \dots, T_{\mathbb{K}}\}$. To assess the relevance of these generated titles, we apply the TextRank algorithm, an unsupervised, graph-based ranking technique. In this approach, we construct a graph $\mathcal{G}=\{\mathcal{T},\mathcal{E}\}$, where each title candidate $T_i \in \mathcal{T}$ is a node in the graph $\mathcal{G}$. 
We initialize an edge between every pair of nodes, with the weight of each edge determined by the cosine similarity between the two corresponding title candidates.
To calculate the cosine similarity between two title candidates, we utilize the Term Frequency and Inverse Document Frequency (TF--IDF) method. We construct a token vocabulary $\mathcal{V}$ from the set of titles $\mathcal{T}$. Each title $T_i$ is represented by a vector $v_{T_i} = {w_1^i, w_2^i,\dots,w_m^i}$, where $m$ is the size of the vocabulary, and $w_j^i$ is calculated as follows:
\begin{equation}
    \label{eq:tf-idf}
    w_j^i = tf_j^i \times idf_j = (\log{f_j^i}+1) \times (\log{\frac{\mathbb{K}}{\mathbb{K}_i}} + 1)
\end{equation}
with $f_j^i$ being the frequency of the $j^{th}$ token in title $T_i$, $\mathbb{K}_i$ as the number of titles that contain this token, and $\mathbb{K}$ being the total number of title candidates. 
The lexical similarity between the TF--IDF vectors of $T_i$ and $T_j$ is computed, as detailed in Equation~\ref{eq:ranking}.
% In this study, we aim to create high-quality titles for \SO post with a specific focus on mitigating the issue of high-variance in generation quality through the use of a post-rankling method at the inference stage.
% For each \SO post input $\mathcal{X}$, the model predicts a set of $n$ title candidates, $\mathcal{T} = \{T_1, T_2, \dots, T_n\}$.
% We utilize the TextRank algorithm~\cite{mihalcea2004textrank}, an unsupervised graph-based ranking method to evaluate the relevance score of generated titles.
% Given a graph $\mathcal{G} = \{\mathcal{T},\mathcal{E}\}$ in which the title candidate $T_i \in \mathcal{T}$ represents the $i^{th}$ node of $\mathcal{G}$.
% The undirected edge $e_{ij} \in \mathcal{E}$ connects two nodes $T_i$ and $T_j$ and is weighted by the cosine similarity between the two title candidates.
\begin{equation}
    \label{eq:ranking}
    Sim(T_i,T_j) = \ell_{ij} =\frac{\overrightarrow{v_{T_i}} \cdot \overrightarrow{v_{T_j}}}{{\lVert\overrightarrow{v_{T_i}}\rVert\times\lVert\overrightarrow{v_{T_j}}\rVert}} 
\end{equation}
where $v_{T_i}$ and $v_{T_j}$ denote the TF--IDF vectors of $T_i, T_j$, respectively.
The TextRank algorithm assigns a relevance score to each node, which is iteratively refined until it converges, as in Equation~\ref{eq:textrank}.
\begin{equation}
    \label{eq:textrank}
    \mathcal{S}_{i} = (1-a) + a \sum\limits_{j \neq i}  \frac{\ell_{ij}}{\sum\limits_{k \neq j}\ell_{jk}}\mathcal{S}_j
\end{equation}
where $a$ represents a damping factor used in the TextRank algorithm, typically set to $0.23$. $\mathcal{S}_i$ and $\mathcal{S}_j$ denote the relevance scores of the $i^{th}$ and $j^{th}$ nodes, respectively.
The title that achieves the maximum relevance score is then selected as the best one.


% \subsection{Pre-trained Language Models}~\label{sec:ptm}

% Theoretically, \tool's methodology including Distribution-Balanced Loss and Low-Confident Filter can be applied for fine-tuning and inference of any Pre-trained Language Models. However, given resource constraints, our work focuses on four well-known PTMs including BERT~\cite{bert}, BART~\cite{lewis2020bart}, RoBERTa~\cite{roberta}, and ELECTRA~\cite{electra}. This section recalls these models in detail. 

% \subsubsection{BERT.}
% (Bidirectional Encoder Representations from Transformers) is a language model developed by Google. It utilizes a bidirectional architecture to understand the context of words by considering both left and right surrounding words simultaneously. The model's training procedure includes two steps: pre-training and fine-tuning. It was pre-trained on a diverse range of datasets, a combination of the BookCorpus~\cite{bookcorpus} plus English Wikipedia, with two objectives: Masked language modeling (MLM) and Next sentence prediction (NSP). In this study, we focus on the original base model of BERT with 110 millions of parameters.

% \subsubsection{BART.} is a denoising autoencoder built with a sequence-to-sequence model developed by Facebook. It is a transformer encoder-decoder with a bidirectional (BERT~\cite{bert}-like) encoder and an auto-regressive (GPT~\cite{gpt1}-like) decoder. BART is pre-trained by corrupting text with an arbitrary noising function and learning a model to reconstruct the original text. The architecture is closely related to that used in BERT, with some differences, and in total, it contains roughly 10\% more parameters than the equivalently sized BERT model.

% \subsubsection{RoBERTa.} (Robustly optimized BERT approach) an improved recipe for training BERT~\cite{bert} model, that can match or exceed the
% performance of all of the post-BERT methods. RoBERTa is trained with dynamic masking, full sentences without NSP loss, large mini-batches, and a larger byte-level BPE. The dataset for training includes five English-language corpora of
% varying sizes and domains including English Wikipedia, OpenWebText,\footnote{\url{https://github.com/jcpeterson/openwebtext}} BookCorpus~\cite{bookcorpus}, and CC-News~\cite{mackenzie2020cc}.

% \subsubsection{ELECTRA.} is a new method for self-supervised language representation learning with little amount of computation. Its models are trained to distinguish ``real'' input tokens vs. ``fake'' input tokens generated by another neural network, similar to the discriminator of a GAN~\cite{gan}.
% ELECTRA includes two neural networks called a generator and a discriminator. Despite the similar structure to GAN, the generator, a small masked language model, is trained with maximum likelihood rather than adversarially. After pre-training, the generator is thrown out and the discriminator is fine-tuned on downstream tasks.


==> src/RelatedWork.tex <==
%\section{Related work \label{sect:related_work}}


In this section, we review notable studies that are relevant to ours. First, we present approaches that perform the multiclassification using \RM and additional textual content in Section \ref{sec:readme}. Afterward, approaches that support the automation of \GH workflows are overviewed in Section \ref{sec:workflows}. 


\subsection{Categorization of \RM files} \label{sec:readme}

%The work of David Lo.

Prana \etal~\cite{DBLP:journals/ese/PranaTTAL19} developed an approach to the categorization of \RM files.

GHTRec~\cite{9590294} predicts the list of topics using the preprocessed \texttt{README} content using the BERT model. Furthermore, the tool suggests the most similar trending repositories, namely the most starred ones, by computing the similarity on the topic vectors mined from the user's historical data. 

Izadi \etal ~\cite{izadi2020topic} exploit a fine-tuned version of the BERT model to classify Github repositories from the textual content. To feed the underpinning model, the training data includes 152K GitHub repositories and 228 featured topics. Afterward, the tool exploits a fine-tuned version of the DistilBERT model to classify the input repository from all the collected textual data, \ie \RM content, project name, descriptions, wiki pages, and file names.  The same authors enrich the proposed classifier by exploiting semantic relationships \cite{izadi_semantically-enhanced_2023}. To this end,  a knowledge graph composed of 2,234 semantic relationships and 863 curated topics has been built according to \textit{(i)} their popularity and \textit{(ii)} the degree in the produced graph. The novel approach, called SED-KG, is eventually employed to enhance the performances of existing recommender systems for GitHub topics.  

HybridRec \cite{di_rocco_hybridrec_2022} predicts a list of GH topics by relying on two components, \ie a stochastic classifier and a collaborative filtering engine. The former is a Complement Naive Bayesian (CNB) network that encodes \RM content using a TF-IDF weighting scheme to predict an initial set of topics. The latter exploits such predictions to infer additional tags, thus increasing the coverage by considering the mutual relationships encoded as a graph. 


ClassifyHub~\cite{soll2017classifyhub} is an ensemble learning approach that relies on the InformatiCup 2017 dataset\footnote{\href{https://github.com/informatiCup/informatiCup2017}{https://github.com/informatiCup/informatiCup2017}} to perform the text classification task.  

GitRanking \cite{sas_gitranking_2023} makes use of the active sampling algorithm for Pairwise comparisons (ASAP) to build a topic taxonomy by combining \RM files and Wikidata definition. After the collection of the training data, manual filtering is applied by involving real developers who annotate the most 3,000 topics. Afterward, the ASAP strategy is used to perform the final ranking by exploiting the WikiData description of each topic. The results show that the produced taxonomy improves the results of state-of-the-art \RM classifiers. 




% Text summarization has gained interests from researchers that various approaches based on NLP techniques have been proposed to solve this task.

% With the dramatic development of machine learning algorithms, automatic text summarization has garnered %become one of the most common problems that gains 
% much attention from the  research community in recent years. 








%\subsection{Summarization} \label{sec:summarization}


\subsection{Specification of \GH workflows by means of actions} \label{sec:workflows}


Mastropaolo \etal \cite{10.1145/3597503.3623351} presented GH-WCOM (GitHub Workflow COMpletion), a Transformer-based approach supporting developers in writing a specific type of CI/CD pipelines, namely GitHub workflows. 

This work~\cite{10.1145/3593434.3593475}.


%
%
%\subsection{Text summarization} \label{sec:TextSummarization}
%
%%\PN{Something about extractive summarization and abstractive summarization.}
%
%Summarization has been conceived as an effective means to generate a shorter but informative summary from long pieces of text \cite{bart2020,t52019}. %This aims to create a concise and coherent summary that only provides the main points of the document. 
%%researchers in NLP community.
%There are two main types of approaches in automatic text summarization, namely extractive summarization and abstractive summarization. %On the one hand, t
%The former involves selecting important keyphrases from the original text and combining them to produce a summary without generating any new text. With various algorithms being proposed, the main tasks have been effectively resolved, including intermediate representation, sentence score, and summary sentence selection \cite{Nenkova2012}. %On the other hand, 
%Meanwhile, the latter entails more deep understanding of the document, which could offer a realistic summary by employing paraphrasing sentences or new text generation %It could overcome the problem of grammar inconsistencies in the extractive approach with the help of advanced natural language techniques~%employing semantic representation, inference, and natural language generation
%\cite{Bahdanau2015,Nenkova2012}.
%
%Extractive summarization has become a trendy research topic with a high level of maturity \cite{GUPTA201949}. Starting with initial ideas based on scoring sentences \cite{Christian2016,Radev2001}, various approaches with the help of neural networks recently have been proposed that show impressive results \cite{ANAND20222141,Mohsen2020}.
%% which indicates that this topic is still in great demand.  
%Now the community has shifted towards abstractive summarization which requires deeper analysis of the input text in order to generate a more human-like summary \cite{GUPTA201949,MOHAN201632,Iwasaki2019,Lee2020,Xu2020}. %With the inspiration of the encoder-decoder architecture, various research has been conducted recently \cite{Iwasaki2019,Lee2020,Xu2020}, showing a potential application in solving different summarization tasks.
%% Besides being believed that this model is smoother, the encoderdecoder framework is also convenient in adjusting parameters automatically (Xu et al., 2020).
%% This is because abstractive summaries are more complex and complicated than extractive summaries. the abstractive summarization needs extensive NLP but more real as human.
%
%%With respect to our study, 
%In this work, we formulate the  generation of descriptions from \RM as an abstractive summarization task. We aim to produce realistic and useful summaries for \GH repositories. %This will provides developers with a practical means to quickly understand a \GH repository. %by means of a succinct summary.  
%
%
%\subsection{Summarization in Software Engineering}
%% \subsection{Summarization for SE artifacts}
%
%% To help developers generate high-quality titles for issues on \GH, 
%% to formulate this problem into a 
%
%Recently, the SE community has deployed summarization in different tasks. %artifacts. %
%%summarization has attracted attention from the SE community. 
%Chen \etal \cite{Chen2020} proposed \IT, an approach to the generation of high-quality titles for issues on \GH, exploiting one-sentence summarization. %They proposed \IT based on a seq2seq model \cite{Sutskever2014} %which could be considered as a specialized tool 
%% to generate title for issue description. 
%% Though \IT yielded a promising performance, 
%Hao \etal \cite{HaoLin2022} %found the ROUGE-L scores of only 42.7\% of titles can exceed 0.3. Therefore, they proposed 
%developed a quality prediction-based filter TitleGen-FL including the deep learning-based (DL) module and the information retrieval-based (IR) module. This filter can predict whether the method iTAPE can generate a high-quality title by analyzing the issue body. %Similary, Zhang \etal \cite{itiger2022} utilized BART to summarize issue titles. %pre-trained model in solving this task. 
%
%% In automatic evaluation, their proposed approach, namely iTIGER, achieves better summarization performance in comparison with iTAPE.
%
%%Since hundreds of various items must be included, producing release notes are considered a time-consuming and daunting task. 
%
%Moreno \etal developed ARENA %(Automatic RElease Notes generAtor) 
%\cite{Moreno2014, Moreno2017}, an approach for the automatic generation of release notes that combines in a unique way source code analysis, code summarization techniques, and information from versioning systems and issue trackers. 
%% At the end, the release note is organized into categories and presented in hierarchical HTML format.
%% In the code summarization step, they perform several processing operators such as (i) hierarchically organizing the code changes; (ii) selecting the changes to be described; and (iii) generating a set of natural-language
%% sentences for the selected changes. 
%The obtained results indicate that ARENA is effective in producing helpful release notes, as considered by professional %and open-source 
%developers. With a different direction, a recent study \cite{DeepRelease2022} introduced an approach named DeepRelease to generate release notes according to pull requests. The approach exploits useful information from pull requests, and then %fits them into a deep-learning model in order to 
%summarizes change entries in release notes effectively.
%
%% Generating high-quality titles for Stack Overflow posts is an ongoing research topic, and 
%% solve this problem as a summary task
%
%
%
%
%
%
%Studies have been conducted to generate titles for Stack Overflow posts. Gao \etal \cite{Gao2020} were the first to automatically generate a post title according to a specific code snippet, %. From their proposed method, they 
%implementing a tool named Code2Que which employs a sequence-to-sequence model as their backbone model. %However, they ignored the valuable information in the corresponding problem description. From this motivation, 
%Liu \etal \cite{Liu2022} considered both modalities (code snippet and problem description) in their work. They proposed SOTitle, which is fine-tuned based on the pre-trained transformer language model T5. The experimental results showed that SOTitle outperforms various baselines including Code2Que. %By combining the pre-trained CodeT5 model and the maximal marginal multiple nucleus sampling strategy, M3NSCT5 \cite{Fengji2022} can generate high-quality and diverse title candidates for the developers to choose.
%
%\RM contains important information about % %features of 
%source code, and it could scale dramatically with large-scale projects. As no studies have tackled the issue of \RM summarization, we conduct this work %has been conducted with the ultimate aim of 
%with the aim of helping developers quickly catch up with a \GH repository by means of a succinct summary.


% summarizes information in README in
% more complete and precise information than the manually produced ones.

% by extracting changes from the source code, summarizing them, and integrating them with information from versioning systems and issue trackers. 
% talk about text summarization in general

% talk about text summarization in software engineering

% release note generation

% issue title generation, itape, itiger, TitleGen-FL,

% post title generation in stack over flow, from Mined Code Snippets


% As noted in the introduction, the ``\verb|acmart|'' document class can
% be used to prepare many different kinds of documentation --- a
% double-blind initial submission of a full-length technical paper, a
% two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
% journal article, a SIGCHI Extended Abstract, and more --- all by
% selecting the appropriate {\itshape template style} and {\itshape
%   template parameters}.

% This document will explain the major features of the document
% class. For further information, the {\itshape \LaTeX\ User's Guide} is
% available from
% \url{https://www.acm.org/publications/proceedings-template}.



==> src/Related_Work.tex <==
\section{RELATED WORK} 
\label{sec:RelatedWork}
%\section{BACKGROUND AND RELATED WORK} 


This section introduces a brief overview on the background of Pre--trained Language Models (PLMs) along with their applications in Software Engineering and the state-of-the-art works for \SO post title generation.

\subsection{Pre-trained Language Models (PLMs)}
Deep learning has witnessed the successful application of the attention mechanism across diverse domains, ranging from image recognition, natural language processing (NLP), recommendation systems~\cite{zhao2020exploring,chaudhari2021attentive}.
The emergence of the Transformer architecture, introduced by Vaswani et al.~\cite{vaswani2017attention}, along with its adept utilization of attention mechanisms, has profoundly impacted the realm of NLP. This pivotal development has marked the onset of a new era for contemporary language representation models such as BERT~\cite{bert}, RoBERTa~\cite{roberta}, GPT-2~\cite{radford2019language}, BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}, and others.
These models share a commonality in employing transfer learning through pre-training, enabling them to acquire a comprehensive language representation from extensive unlabeled data, which can subsequently be fine-tuned for diverse downstream tasks~\cite{howard2018universal}. 
For instance, BERT~\cite{bert}, leveraging the encoder of the Transformer, proves to be a versatile Pre-trained Language Model (PLM) applicable in diverse downstream tasks like text similarity~\cite{tracz2020bert} and text classification~\cite{garg2020bae}. 
On the other hand, GPT-2~\cite{radford2019language}, relying on the Transformer’s decoder, excels in natural language generation problems~\cite{peng2020few}.
Lewis et al. introduced the BART model~\cite{lewis2020bart}, which incorporates both auto-regressive and bi-directional training objectives during pre-training, showcasing proficiency in diverse sequence-to-sequence tasks including document summarization, text generalization~\cite{akiyama2021hie}.
More recently, the T5 model~\cite{raffel2020exploring}, presented as a unified text-to-text PLM, consistently demonstrates state-of-the-art performance across tasks ranging from classification to generalization~\cite{zhuang2023rankt5}.
%PLMs for code
Apart from PLMs tailored for NLP tasks, research is increasingly focusing on Pre-trained Code and Language Models (PCLMs) to address programming language-related tasks. 
%like code summarization, API recommendation, code completion, and others. 
PCLMs, trained on code repositories, include diverse models such as CodeBERT~\cite{feng2020codebert}, PLBART~\cite{ahmad2021unified}, UnixCoder~\cite{guo2022unixcoder}, CodeT5~\cite{wang2021codet5}, and others.

Harnessing the substantial capabilities of PLMs and PCLMs, various studies have employed these models, achieving promising results in numerous Software Engineering (SE) tasks, including code summarization~\cite{ahmad2021unified,shi2022natural,zhou2022automatic}, program analysis~\cite{huang2022prompt}, code generation~\cite{liu2023refining}, to name a few. %and others.
Within these tasks, our study aligns most closely with the utilization of PLMs for code summarization~\cite{ahmad2021unified,shi2022natural,zhou2022automatic} and natural language-based text summarization in SE tasks, such as GitHub dialog summarization~\cite{fan2023dialog} and pull-request title generation~\cite{irsan2022autoprtitle,zhang2022automatic}.
Fan et al.~\cite{fan2023dialog} proposed ADSum, utilizing a fine-tuned T5 model to analyze GitHub discussion posts and generate summaries for annotators. 
They introduced the prompt-tuning technique to leverage few-shot annotated data for producing high-quality summarization of the dialog.
Zhang et al.~\cite{zhang2022automatic} have introduced the task of automatic generation of pull request titles for GitHub repositories using pre-trained baseline models, such as BERTSumExt~\cite{liu2019text}, BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}.% and others. 

%to the specialized field of software engineering~\cite{vaswani2017attention,von2022validity,li2023pre}.
%Pre-trained Language Models (PLMs), exemplified by BERT~\cite{bert}, RoBERTa~\cite{roberta}, BART~\cite{lewis2020bart}, T5~\cite{raffel2020exploring}, and others, rely typically on the Transformer architecture, pioneered by Vaswani et al.~\cite{vaswani2017attention}, particularly leveraging attention mechanisms for their effectiveness and success in various research domains.
%These models are trained on extensive datasets, enabling them to grasp both the syntax and semantics of natural languages.






\subsection{Title Generation for \SO posts}
\SO (SO) serves as a widely used Question-Answering platform where software developers can seek solutions to programming-related queries. Mondal et al.~\cite{mondal2021early} highlighted that an increasing number of open questions on SO remain unanswered, partially attributed to the suboptimal quality of the question expression. Numerous research endeavors have been dedicated to addressing this issue, with a specific focus on crafting high-quality question titles~\cite{gao2021code2que,zhang2022improving,liu2023automated,zhang2023diverse,liu2022sotitle,zhou2023qtc4so}.
These investigations predominantly revolved around generating question titles by analyzing the content of SO posts, including problem descriptions and code snippets.

%code snippets to title - code summarization
Initial studies in this domain depended solely on code snippets for generating question titles, aligning closely with the code summarization task~\cite{tang2022ast,cheng2022keyword,shi2022natural,zhou2022automatic}. 
The concept of code summarization was initially conceived as a specialized Programming Language-to-Natural Language translation task, employing the sequence-to-sequence architecture within the encoder-decoder paradigm~\cite{ahmad2021unified}.
Building on this foundation, Gao et al.\cite{gao2021code2que} introduced Code2Que to generate Stack Overflow titles. This model employs bi-directional LSTMs, coupled with an attention mechanism, to encode the sequence of code tokens into hidden states, subsequently decoding them into concise question titles in natural language. 
This method also incorporated two conventional Natural Language Processing (NLP) techniques. It implemented a coverage mechanism~\cite{tu2016modeling} to mitigate word repetition issues and a copy mechanism~\cite{gu2016incorporating} to address out-of-vocabulary challenges.
Despite Code2Que exhibiting promising performance, LSTMs may struggle to handle long-range dependencies, leading to challenges in capturing the semantic meaning of the entire source code.
The most recent research efforts seek to harness the extensive dataset for pre-training language models and then fine-tuning for a specific task, resulting in state-of-the-art achievements, particularly in code summarization~\cite{ahmad2021unified,guo2022unixcoder} and SO post title generation~\cite{zhang2023diverse}.
Ahmad et al.~\cite{ahmad2021unified} introduced the Transformer model to tasks related to programming languages such as code summarization, code generation and code translation.
They proposed PLBART with the use of pairwise position encoding to capture the long-range dependencies among code tokens.
Subsequent studies focus on introducing multilingual representation models tailored for programming languages, as exemplified by UnixCoder~\cite{guo2022unixcoder}, CodeT5~\cite{wang2021codet5}.
Zhang et al.~\cite{zhang2023diverse} introduced M3NSCT5, fine-tuning the CodeT5 model to translate code sequences into relevant titles for Stack Overflow posts. 
However, the lack of context around code snippets can lead to the same code snippets being associated with different titles, introducing ambiguity. 
In addressing this, M3NSCT5
%their method \textbf{DAVIDE: WHICH ONE?} 
emphasizes diversifying generated texts using Nucleus Sampling strategy~\cite{holtzman2019curious} and Maximal Marginal Ranking~\cite{yang2021maximizing}, providing users with a selection of titles for a given code snippet.
While our approach shares the aspect of producing multiple candidates during the inference stage, our primary goal differs – we aim to identify the most relevant title aligned with the input question description and code snippets.

%(description + code snippets) to title - abstractive text summarization
Zhang et al.~\cite{zhang2022improving} have shown that incorporating both the problem description and code snippets contributes to clarifying the context, enhancing the clarity, and improving the completeness of question titles.
Recent studies in the realm of code summarization have also recognized that the inclusion of additional information, such as API documentation~\cite{hu2018summarizing}, source code comments~\cite{wei2020retrieve}, alongside the source code, has demonstrated improved performance compared to relying solely on the source code.
Pre-trained Language Models with the ability of multi-modal input modelling are typically adopted in these studies.
Zhang et al.~\cite{zhang2022improving} have introduced CCBERT, which leverages the pre-trained CodeBERT model~\cite{feng2020codebert} to parse bi-modal contents (i.e., problem description and code snippets), incorporated with the copy mechanism~\cite{gu2016incorporating} to handle rare tokens.
Liu et al.~\cite{liu2022sotitle} also incorporate multi-modal modeling in their approach, presenting SOTitle for generating Stack Overflow post titles.

SOTitle is constructed upon the pre-trained T5 model~\cite{raffel2020exploring}, aiming to establish a unified model for concurrent training across multiple programming languages. Subsequent research endeavors have adopted this input representation approach for Stack Overflow post title generation~\cite{zhang2023diverse,liu2023automated,zhou2023qtc4so}.
Instead of creating new titles for SO posts, Liu et al.~\cite{liu2023automated} focus on reformulating question titles through the analysis of modification logs on the Stack Overflow platform.
The proposed QETRA model also employs the pre-trained T5 as the backbone model to learn the title reformulation patterns from the extracted title modification logs.
In contrast to previous research, QETRA employs both the question body (comprising code snippets and problem description) and the question titles provided by users to suggest candidate reformulated titles.
Another task closely related to the generation of Stack Overflow post titles is the completion of question titles.
Zhou et al.~\cite{zhou2022automatic} introduced QTC4SO, an innovative approach for generating Stack Overflow post titles from bi-modal post contents and incomplete titles. Utilizing the pre-trained T5 model, QTC4SO learns potential title completion patterns and incorporates a multi-task learning strategy to leverage meaningful information from various programming languages.




%paragraph{The Application of PLMs in Software Engineering}




% This section introduces a brief overview of the background and related works. First, we present recent studies on the problem of topic recommendation for GitHub repositories. Subsequently, we delve into Large Language Models (LLMs) and their applications for Software Engineering Tasks.

% \subsection{Topic Recommendation for GitHub Repositories}
% \GH topic recommendation is related to %the problem of 
% suggesting relevant topics to repositories on GitHub. In this section, we first recall state-of-the-art techniques for this topic, and then introduce our problem formulation.

% \subsubsection{State-of-the-arts.} Recent approaches in \GH topic recommendation falls into two main categories.

% \vspace{1mm}

% \noindent \textbf{Probability-based Recommendation:} Recommenders based on probability \cite{di2020multinomial, di2022hybridrec, di2020topfilter}, formulate this problem as \textit{multi-class classification} and then employ algorithms, such as Multinomial Naïve Bayesian~\cite{di2020multinomial} to output probability that indicate how likely a topic belong to \GH repository. Particularly, given these probabilities, these techniques rank topics to offer recommendations. In this work, we exclude probability-based techniques such as MNBN~\cite{di2020multinomial} as they have been proven to be less effective than the multi-label-based approaches described below. 

% \vspace{1mm}

% \noindent \textbf{Multi-label Classification:} In contrast to the aforementioned approaches, Izadi et al. \cite{izadi2021topic} recently formalized the GitHub repository topic recommendation task as a \textit{multi-label classification} problem \cite{herrera2016multilabel}. They conducted empirical studies exploring various combinations of (1) document representation and (2) multi-label classification. Their experiments highlighted Logistic Regression with TF-IDF embeddings as the superior combination for topic recommendation, outperforming probability-based recommendation approaches~\cite{izadi2021topic}. Widyasari et al.~\cite{widyasari2023topic} further explores this direction by considering user-defined topics, formulating this problem as an extreme multi-label classification problem. Then, they conducted an exploration study to examine the effectiveness of XML techniques and found that ZestXML~\cite{zeroshotxml} is the best-performing approach in suggesting \GH topics. 

% \subsubsection{Problem Formulation.}
% In this work, we focus on \GH featured topics, which are
% carefully designed and maintained by \GH and its community, following Izadi \etal~\cite{izadi2021topic} as user-defined \GH topics may be noisy and of low quality. However, as rare topics may be still correct and important, we follow Widyasari~\cite{widyasari2023topic} to not remove them. This allows us to ensure both the quality of our dataset and the reliability of the recommendation systems produced in this study. As a result, we obtained a dataset of 665 unique topics (see Section~\ref{sec:dataset}). %Therefore, w
% We formulate our task as a multi-label classification problem, formally explained as follows. %We formally formulate the problem as follow:

% \vspace{1mm}

% \noindent \textbf{Prior Knowledge.} A labelled dataset $\mathcal{D} = (\mathcal{G}, \mathcal{T}, \mathcal{M})$, where $\mathcal{G}$ is set of GitHub repositories and $\mathcal{T}$ is set of featured topics. $\mathcal{M}$ is a mapping from $\mathcal{G}$ to set of subsets of $\mathcal{T}$, where $\mathcal{M}(g) \subseteq \mathcal{T}$ is the set of topics for a GitHub repository $g$.

% \vspace{1mm}

% \noindent \textbf{Input.}  A new (unlabelled) dataset $\mathcal{D}_{new} = (\mathcal{G}_{new}, \mathcal{T}_{new})$ where $\mathcal{G}_{new} \neq \mathcal{G}$ is a set of  repositories and $\mathcal{T}_{new} \supseteq \mathcal{T}$ is set of labels. We consider the repositories' descriptions and README files in this study.

% \vspace{1mm}

% \noindent \textbf{Output.} A mapping $\mathcal{M}_{new}$ from $\mathcal{G}_{new}$ to set of subsets of $\mathcal{T}_{new}$ such that $\mathcal{M}_{new}(g) \subseteq \mathcal{T}_{new}$ is the set of labels for each repository $g \in \mathcal{G}_{new}$.


% \subsection{Pre-trained Language Models}
% Pre-trained Language Models (PTMs) ~\cite{bert, roberta, lewis2020bart, electra} become popular in many domains including Natural Language Processing and Software Engineering thanks to their remarkable capabilities. These models are commonly built based on a Transformer architecture~\cite{vaswani2017attention} and trained on a massive amount of data, allowing them to learn and capture both the syntax and semantics of human language. Given these capabilities, PTMs showed excellent performance in extracting semantic features from textual data and great promise to be fine-tuned for tasks that they were not initially trained for~\cite{min2023recent, yang2022aspect, hou2023large, nguyen2023multi, zhang2020sentiment}.

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=0.69\textwidth]{img/TopicRecommend.pdf}
%     \caption{Overall workflow of \tool.}
%     \label{fig:overview}
% \end{figure*}

% Inspired by these successes, PTMs have been widely adopted in Software Engineering tasks such as code generation~\cite{wang2021codet5, liu2023refining, chen2021evaluating}, program analysis~\cite{huang2022prompt, le2022autopruner, chow2023beware}, and program understanding/reasoning~\cite{ahmed2022few, le2023invalidator, wang2022bridging}. Among these tasks, the applications of PTMs for Natural Language-based Software Engineering (NLBSE) tasks are most closely to our study. Zhang \etal~\cite{zhang2020sentiment} investigated the capabilities of PTMs on sentiment analysis for Software Engineering. He \etal~\cite{he2022ptm4tag} showed the potential of PTMs for recommending tags in Stack Overflow posts. Wang \etal~\cite{wang2021well} proposed the use of PTMs for labeling \GH issues. Messaoud ~\cite{messaoud2022duplicate} applied PTMs for detecting duplicated bug reports. PTMs have been also applied to various other NLBSE tasks such as requirement classification~\cite{luo2022prcbert}, README simplication~\cite{gao2023evaluating}, Software Q\&A~\cite{xu2023we, yang2022answer}. Different from these works, our work delves into the problem of \GH Topic Recommendation. We also investigate challenges, \eg long-tailed distributions for applying PTMs on these tasks, and propose effective mechanisms for handling these challenges. 

% % First paragraph: Introduce about LLM and its capabilities

% % Second paragraph: Present applications of LLM for SE Tasks, e.g., Technical Q&A, Code Summarization, Code Generation, ...

==> src/result/result_code.tex <==
\begin{table}
\caption{Classification Report for 	C$_2$.}
\label{table:classification_code}
\scriptsize
\centering
\begin{tabular}{|l | c| c | c | r |} \hline
	Category & Precision & Recall & F-score & Support\\ \hline
%	\midrule
	AI Assisted & 1.00 & 0.20 & 0.33 & 5\\
	API management & 0.50 & 0.07 & 0.12 & 14\\
	Backup Utilities & 1.00 & 0.50 & 0.67 & 2\\
	Chat & 0.84 & 0.57 & 0.68 & 37\\
	Code Scanning Ready & 1.00 & 0.33 & 0.50 & 3\\
	Code quality & 0.75 & 0.81 & 0.78 & 123\\
	Code review & 0.71 & 0.65 & 0.68 & 97\\
	Code search & 1.00 & 0.17 & 0.29 & 6\\
	Community & 0.50 & 0.05 & 0.08 & 22\\
	Container CI & 0.50 & 0.09 & 0.15 & 56\\
	Continuous integration & 0.89 & 0.94 & 0.91 & 407\\
	Dependency management & 0.75 & 0.57 & 0.65 & 82\\
	Deployment & 0.77 & 0.81 & 0.79 & 189\\
	Desktop tools & 1.00 & 0.10 & 0.18 & 10\\
	GitHub Sponsors & 1.00 & 0.50 & 0.67 & 2\\
	IDEs & 1.00 & 0.17 & 0.29 & 6\\
	Learning & 1.00 & 0.33 & 0.50 & 3\\
	Localization & 1.00 & 0.33 & 0.50 & 3\\
	Mobile & 1.00 & 0.20 & 0.33 & 5\\
	Mobile CI & 1.00 & 0.25 & 0.40 & 8\\
	Monitoring & 1.00 & 0.07 & 0.13 & 14\\
	Open Source management & 0.51 & 0.32 & 0.39 & 75\\
	Project management & 0.60 & 0.40 & 0.48 & 75\\
	Publishing & 0.74 & 0.54 & 0.62 & 145\\
	Reporting & 0.69 & 0.50 & 0.58 & 36\\
	Security & 0.67 & 0.35 & 0.46 & 34\\
	Support & 1.00 & 0.08 & 0.15 & 12\\
	Testing & 0.80 & 0.80 & 0.80 & 100\\
	Time tracking & 1.00 & 0.50 & 0.67 & 2\\
	Utilities & 0.86 & 0.92 & 0.89 & 383\\ \hline
%	\midrule
	micro avg & 0.80 & 0.71 & 0.75 & 1,956\\
	macro avg & 0.84 & 0.40 & 0.49 & 1,956\\
	weighted avg & 0.79 & 0.71 & 0.72 & 1,956\\
	avg & 0.72 & 0.62 & 0.65 & 1,956\\ \hline
\end{tabular}
\end{table}

==> src/result/result_code_comments.tex <==
\begin{table}
\caption{Classification Report for C$_3$.}
\scriptsize
\label{table:classification_code_comment}
\centering
\begin{tabular}{|l | c| c | c | r |} \hline
Category & Precision & Recall & F-score & Support\\ \hline
%\midrule 
AI Assisted & 1.00 & 1.00 & 1.00 & 1\\
API management & 1.00 & 1.00 & 1.00 & 1\\
Backup Utilities & 1.00 & 1.00 & 1.00 & 1\\
Chat & 1.00 & 1.00 & 1.00 & 1\\
Code Scanning Ready & 1.00 & 1.00 & 1.00 & 1\\
Code quality & 0.44 & 0.88 & 0.58 & 8\\
Code review & 0.50 & 0.25 & 0.33 & 8\\
Code search & 1.00 & 1.00 & 1.00 & 1\\
Community & 1.00 & 1.00 & 1.00 & 1\\
Container CI & 1.00 & 0.25 & 0.40 & 4\\
Continuous integration & 0.44 & 0.67 & 0.53 & 30\\
Dependency management & 0.10 & 0.33 & 0.15 & 3\\
Deployment & 0.70 & 0.33 & 0.45 & 21\\
Desktop tools & 1.00 & 1.00 & 1.00 & 1\\
GitHub Sponsors & 1.00 & 1.00 & 1.00 & 1\\
IDEs & 1.00 & 1.00 & 1.00 & 1\\
Learning & 1.00 & 1.00 & 1.00 & 1\\
Localization & 1.00 & 0.50 & 0.67 & 2\\
Mobile & 1.00 & 1.00 & 1.00 & 1\\
Mobile CI & 1.00 & 1.00 & 1.00 & 1\\
Monitoring & 1.00 & 1.00 & 1.00 & 1\\
Open Source management & 0.25 & 0.20 & 0.22 & 5\\
Project management & 0.20 & 0.25 & 0.22 & 4\\
Publishing & 0.50 & 0.21 & 0.30 & 19\\
Reporting & 1.00 & 0.50 & 0.67 & 2\\
Security & 1.00 & 0.33 & 0.50 & 3\\
Support & 1.00 & 1.00 & 1.00 & 1\\
Testing & 0.50 & 0.20 & 0.29 & 5\\
Time tracking & 1.00 & 1.00 & 1.00 & 1\\
Utilities & 0.38 & 0.48 & 0.43 & 31\\ \hline
%\midrule
micro avg & 0.48 & 0.49 & 0.49 & 161\\
macro avg & 0.80 & 0.71 & 0.72 & 161\\
weighted avg & 0.55 & 0.49 & 0.48 & 161\\
avg & 0.39 & 0.33 & 0.34 & 161\\ \hline
\end{tabular}
\end{table}

==> src/result/result_code_statements.tex <==
\begin{table}
\caption{Classification Report for C$_4$.}
\label{table:classification_code_statements}
\scriptsize
\centering
\begin{tabular}{|l | c| c | c | r |} \hline
	Category & Precision & Recall & F-score & Support\\ \hline
%	\midrule 
	AI Assisted & 1.00 & 0.20 & 0.33 & 5\\
	API management & 1.00 & 0.07 & 0.13 & 14\\
	Backup Utilities & 1.00 & 0.50 & 0.67 & 2\\
	Chat & 0.83 & 0.65 & 0.73 & 37\\
	Code Scanning Ready & 1.00 & 0.33 & 0.50 & 3\\
	Code quality & 0.76 & 0.81 & 0.78 & 123\\
	Code review & 0.74 & 0.69 & 0.71 & 97\\
	Code search & 1.00 & 0.17 & 0.29 & 6\\
	Community & 1.00 & 0.09 & 0.17 & 22\\
	Container CI & 0.59 & 0.18 & 0.27 & 56\\
	Continuous integration & 0.87 & 0.95 & 0.91 & 407\\
	Dependency management & 0.73 & 0.59 & 0.65 & 82\\
	Deployment & 0.75 & 0.84 & 0.79 & 189\\
	Desktop tools & 1.00 & 0.10 & 0.18 & 10\\
	GitHub Sponsors & 1.00 & 0.50 & 0.67 & 2\\
	IDEs & 1.00 & 0.17 & 0.29 & 6\\
	Learning & 1.00 & 0.33 & 0.50 & 3\\
	Localization & 1.00 & 0.33 & 0.50 & 3\\
	Mobile & 1.00 & 0.20 & 0.33 & 5\\
	Mobile CI & 1.00 & 0.12 & 0.22 & 8\\
	Monitoring & 0.50 & 0.07 & 0.12 & 14\\
	Open Source management & 0.55 & 0.29 & 0.38 & 75\\
	Project management & 0.62 & 0.32 & 0.42 & 75\\
	Publishing & 0.67 & 0.54 & 0.60 & 145\\
	Reporting & 0.68 & 0.53 & 0.59 & 36\\
	Security & 0.60 & 0.35 & 0.44 & 34\\
	Support & 1.00 & 0.08 & 0.15 & 12\\
	Testing & 0.89 & 0.80 & 0.84 & 100\\
	Time tracking & 1.00 & 0.50 & 0.67 & 2\\
	Utilities & 0.86 & 0.91 & 0.88 & 383\\ \hline
%	\midrule
	micro avg & 0.80 & 0.71 & 0.75 & 1,956\\
	macro avg & 0.85 & 0.41 & 0.49 & 1,956\\
	weighted avg & 0.79 & 0.71 & 0.72 & 1,956\\
	avg & 0.73 & 0.63 & 0.65 & 1,956\\ \hline
\end{tabular}
\end{table}

==> src/result/result_mnb.tex <==
\begin{table}
\caption{Classification Report for CNBN.}
\scriptsize
\label{table:classification_mnb}
\centering
\begin{tabular}{|l | c| c | c | r |} \hline
	Category & Precision & Recall & F-score & Support\\ \hline
%	\midrule
	AI Assisted & 0.25 & 0.33 & 0.29 & 3\\
	API management & 0.20 & 0.06 & 0.09 & 17\\
	Backup Utilities & 0.00 & 0.00 & 0.00 & 2\\
	Chat & 0.61 & 0.94 & 0.74 & 33\\
	Code Scanning Ready & 0.12 & 0.50 & 0.20 & 2\\
	Code quality & 0.64 & 0.81 & 0.71 & 130\\
	Code review & 0.46 & 0.43 & 0.44 & 112\\
	Code search & 0.50 & 0.12 & 0.20 & 8\\
	Community & 0.67 & 0.20 & 0.31 & 30\\
	Container CI & 0.56 & 0.45 & 0.50 & 60\\
	Continuous integration & 0.56 & 0.61 & 0.58 & 392\\
	Dependency management & 0.56 & 0.43 & 0.48 & 91\\
	Deployment & 0.47 & 0.47 & 0.47 & 199\\
	Desktop tools & 0.33 & 0.10 & 0.15 & 10\\
	GitHub Sponsors & 1.00 & 0.50 & 0.67 & 2\\
	IDEs & 0.50 & 0.17 & 0.25 & 6\\
	Learning& 0.00 & 0.00 & 0.00 & 3\\
	Localization & 1.00 & 0.20 & 0.33 & 5\\
	Mobile & 1.00 & 0.25 & 0.40 & 4\\
	Mobile CI & 0.20 & 0.12 & 0.15 & 8\\
	Monitoring & 0.56 & 0.33 & 0.42 & 15\\
	Open Source management & 0.31 & 0.44 & 0.36 & 73\\
	Project management & 0.39 & 0.61 & 0.48 & 77\\
	Publishing & 0.47 & 0.65 & 0.55 & 141\\
	Reporting & 0.31 & 0.29 & 0.30 & 45\\
	Security & 0.40 & 0.21 & 0.27 & 39\\
	Support & 1.00 & 0.10 & 0.18 & 10\\
	Testing & 0.38 & 0.55 & 0.45 & 86\\
	Time tracking & 0.50 & 0.50 & 0.50 & 2\\
	Utilities & 0.53 & 0.48 & 0.50 & 351\\ \hline
%	\midrule
	micro avg & 0.50 & 0.52 & 0.51 & 1,951\\
	macro avg & 0.52 & 0.39 & 0.39 & 1,951\\
	weighted avg & 0.51 & 0.52 & 0.50 & 1,951\\
	avg & 0.49 & 0.52 & 0.50 & 1,951\\ \hline
\end{tabular}
\end{table}

==> src/result/result_text.tex <==
\begin{table}
\caption{Classification Report C$_5$.}
\label{table:classification_text}
\scriptsize
\centering
\begin{tabular}{|l | c| c | c | r |} \hline
	Category & Precision & Recall & F-score & Support\\ \hline
%	\midrule
	AI Assisted & 1.00 & 0.20 & 0.33 & 5\\
	API management & 1.00 & 0.07 & 0.13 & 14\\
	Backup Utilities & 1.00 & 0.50 & 0.67 & 2\\
	Chat & 0.82 & 0.62 & 0.71 & 37\\
	Code Scanning Ready & 1.00 & 0.33 & 0.50 & 3\\
	Code quality & 0.80 & 0.81 & 0.80 & 129\\
	Code review & 0.73 & 0.64 & 0.68 & 103\\
	Code search & 1.00 & 0.12 & 0.22 & 8\\
	Community & 1.00 & 0.04 & 0.08 & 25\\
	Container CI & 0.50 & 0.09 & 0.15 & 58\\
	Continuous integration & 0.85 & 0.94 & 0.89 & 432\\
	Dependency management & 0.76 & 0.61 & 0.68 & 89\\
	Deployment & 0.75 & 0.84 & 0.79 & 194\\
	Desktop tools & 1.00 & 0.10 & 0.18 & 10\\
	GitHub Sponsors & 1.00 & 0.50 & 0.67 & 2\\
	IDEs & 1.00 & 0.17 & 0.29 & 6\\
	Learning & 1.00 & 0.33 & 0.50 & 3\\
	Localization & 1.00 & 0.25 & 0.40 & 4\\
	Mobile & 1.00 & 0.20 & 0.33 & 5\\
	Mobile CI & 0.50 & 0.11 & 0.18 & 9\\
	Monitoring & 0.50 & 0.07 & 0.12 & 15\\
	Open Source management & 0.49 & 0.31 & 0.38 & 78\\
	Project management & 0.65 & 0.42 & 0.51 & 76\\
	Publishing & 0.64 & 0.49 & 0.56 & 149\\
	Reporting & 0.66 & 0.53 & 0.58 & 36\\
	Security & 0.67 & 0.38 & 0.48 & 37\\
	Support & 1.00 & 0.08 & 0.15 & 12\\
	Testing & 0.83 & 0.83 & 0.83 & 102\\
	Time tracking & 1.00 & 0.50 & 0.67 & 2\\
	Utilities & 0.86 & 0.90 & 0.88 & 402\\ \hline
%	\midrule
	micro avg & 0.79 & 0.71 & 0.75 & 2,047\\
	macro avg & 0.83 & 0.40 & 0.48 & 2,047\\
	weighted avg & 0.78 & 0.71 & 0.71 & 2,047\\
	avg & 0.71 & 0.61 & 0.64 & 2,047\\ \hline
\end{tabular}
\end{table}
